DistilHuBERT: Speech Representation Learning by Layer-wise Distillation of Hidden-unit BERT

Self-supervised speech representation learning methods like wav2vec 2.0 and Hidden-unit BERT (HuBERT) leverage unlabeled speech data for pre-training and offer good representations for numerous speech processing tasks. Despite the success of these methods, they require large memory and high pre-training costs, making them inaccessible for researchers in academia and small companies. Therefore, this paper introduces DistilHuBERT, a novel multi-task learning framework to distill hidden representations from a HuBERT model directly. This method reduces HuBERT's size by 75% and 73% faster while retaining most performance in ten different tasks. Moreover, DistilHuBERT required little training time and data, opening the possibilities of pre-training personal and on-device SSL models for speech.

==> figure/hubert.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.72\linewidth]{figure/HuBERT_model.pdf}
    \vspace*{-10pt}
    \caption{
        HuBERT \cite{hsu2021hubert}.
        MSK denotes masked frames.
    }
    \label{fig:hubert}
    \vspace*{-10pt}
\end{figure}

==> table/batch.tex <==
\begin{table}[t]
    \caption{
        Pre-training with different batch sizes.
    }
    \vspace{4pt}
    \label{tab:batch}
    \centering
    \begin{tabular}{lcccc}
        \toprule
        &  & IC & SID & ASR \\
        \cmidrule{3-5}
        Batch Size & Updates & Acc$\uparrow$ & Acc$\uparrow$ & WER$\downarrow$ \\
        \midrule
        6 & 800k & 94.20 & 68.03 & 12.71 \\
        24 & 200k & 94.17 & 72.83 & 13.26 \\
        48 & 100k & 93.28 & 70.61 & 13.93 \\
        \bottomrule
    \end{tabular}
\end{table}
